One-Shot Sensitivity-Aware Mixed Sparsity Pruning for Large Language Models

Various Large Language Models~(LLMs) from the Generative Pretrained Transformer(GPT) family have achieved outstanding performances in a wide range of text generation tasks. However, the enormous model sizes have hindered their practical use in real-world applications due to high inference latency. Therefore, improving the efficiencies of LLMs through quantization, pruning, and other means has been a key issue in LLM studies. In this work, we propose a method based on Hessian sensitivity-aware mixed sparsity pruning to prune LLMs to at least 50% sparsity without the need of any retraining. It allocates sparsity adaptively based on sensitivity, allowing us to reduce pruning-induced error while maintaining the overall sparsity level. The advantages of the proposed method exhibit even more when the sparsity is extremely high. Furthermore, our method is compatible with quantization, enabling further compression of LLMs. We have released the available code.

==> sections/related_work.tex <==
\subsection{Post-training Pruning}
% Post-training Pruning通常是这样一个场景，我们被给予了一个训练收敛的模型\theta，和一些校准数据c，这些校准数据通常是非常少的小批量数据。通过一些模型压缩技术(例如量化和剪枝)将\theta压缩到一个紧凑的版本\theta^*。这种场景最初是来源于量化中的PTQ，后来推广到了剪枝的领域。
% TODO：THIS SECTION SHOULD BE UNDER METHODOLOGY, NOT RELATED WORK
Post-training pruning typically involves a scenario where we are provided with a training-converged model $\theta$ and some calibration data \textsc{c}. This calibration data often consists of a very limited amount of small-batch data.
By employing certain model compression techniques (such as quantization and pruning), $\theta$ is compressed into a compact version $\theta^*$. This scenario initially emerged within the context of post-training quantization and later extended to the field of pruning.

\begin{equation}
    \theta^* = \texttt{Pruner}(\theta, \textsc{c}),
\end{equation}
\begin{equation}
    L_{prun} = ||\theta^*(\mathit{X}) - \theta(X)||_2^2,
\end{equation}
where \texttt{Pruner} is a pruning method, \textit{X} represents the input, and $L_{prun}$ stands for compression error. Our objective is to minimize the compression error in this context.

% 基于OBS的Mask Selection和权重重构
\subsection{Mask Selection and Weight Reconstruction Based on OBS}
% SparseGPT中通过使用传统方法OBS进行求解模型剪枝后权重的更新问题，对于未剪枝的权重W，要使得剪枝后得到的最优的权重W^*满足等式\eqref{3}。对于\eqref{6}中要使得E(\delta W)最小，可以通过最小二乘法和拉格朗日乘值法求得最优解。OBS更新在等式\eqref{7}中的$\delta W$提供了剩余权重的最优调整，以补偿在索引m处去除权重的影响，会导致剪枝带来的误差为\eqref{8}中的$\varepsilon_m$。
% 当第m行的权重元素更新量为等式\eqref{7}中的$\delta W_m$时，可以使得剪枝误差最小，并带来\eqref{8}中的$\varepsilon_m$的剪枝误差量。
In SparseGPT~\cite{Frantar_Alistarh_2023}, the weight update problem after model pruning is solved using the traditional method OBS\cite{Hassibi_Stork_1992}. For the ORIGINAL weights $W$, the objective is to ensure that the optimized pruned weights $W^*$ satisfy equation \eqref{eq:eq1}. To minimize $E(\delta W)$ in equation \eqref{eq:eq2}, WE employ Taylor expansion. 

TODO: USE MEANINGFUL TAGS TO INDICATE EQUATIONS, NOT BY EQ1 EQ2 ETC.
% By solving for the case where the weight element in the m-th row is updated to $\delta W_m$ as in equation \eqref{eq:eq3}, you achieve the minimal pruning error, resulting in the pruning error quantity \(\varepsilon_m\) as indicated in equation \eqref{eq:eq4}.
The update of OBS, in equation \eqref{eq:eq3}, provides the optimal adjustment of the remaining weights, denoted as $\delta W$, to compensate for the impact of weight removal at $m$-th row. This impact is responsible for the error introduced by pruning, as indicated by $\varepsilon_m$ in equation \eqref{eq:eq4}.
\begin{equation}
\label{eq:eq1}
    W^* = \arg \min_{\hat{W}}||WX-\hat{W}X||_2^2,
\end{equation}
where $W^*$ denotes the optimally pruned weights, W represents the initial weights, and X is the input.
\begin{equation}
\label{eq:eq2}
    E(\delta W) = ||WX-(W+\delta W)X||_2^2,
\end{equation}
where $\delta W = W^* - W$ and $E(\delta W)$ represents the expected pruning-induced error.
\begin{equation}
\label{eq:eq3}
    \delta W_m = - \frac{w_m}{[H^{-1}]_{mm}}·H^{-1}_{:,m},
\end{equation}
\begin{equation}
\label{eq:eq4}
   \varepsilon_m = \frac{w^2_m}{[H^{-1}]_{mm}},
\end{equation}
where $w_m$ represents the original weight elements of the m-th row. $H = XX^T$, where $H^{-1}$ denotes the inverse matrix of $H$.
% $w_m$是第m行的原始权重元素，$H=X*X^T$, $H^{-1}$表示H的逆矩阵。
% 我们以$\varepsilon_m$作为第m行元素的显著性指标，通过对它进行从小到大的排序，选取前p\%（p为稀疏度）的元素作为被剪枝的元素，并把选取元素对应的索引在mask $M_m$中置为0，其余置为1。通过eq.\eqref{eq:eq5}对权重进行剪枝。
\begin{equation}
\label{eq:eq5}
    W_m^* = M_m \ \begin{tikzpicture}
  \draw (0,0) circle (0.12cm);
  \fill (0,0) circle (1.0pt);
\end{tikzpicture} \ W,
\end{equation}

We utilize $\varepsilon_m$ as the saliency criterion for the $m$-th row elements. By sorting them in ascending order, we select the top $p\%$ (where $p$ represents the sparsity level) of elements as candidates for pruning. The corresponding indices of these selected elements are then set to 1 in the mask $M_m$, while the rest are set to 0. Pruning of the weights is performed using equation \eqref{eq:eq5}.
